Properties of Reddit News Topical Interactions

Most models of information diffusion online rely on the assumption that pieces of information spread independently from each other. However, several works pointed out the necessity of investigating the role of interactions in real-world processes, and highlighted possible difficulties in doing so: interactions are sparse and brief. As an answer, recent advances developed models to account for interactions in underlying publication dynamics. In this article, we propose to extend and apply one such model to determine whether interactions between news headlines on Reddit play a significant role in their underlying publication mechanisms. After conducting an in-depth case study on 100,000 news headline from 2019, we retrieve state-of-the-art conclusions about interactions and conclude that they play a minor role in this dataset.

==> table-MPDHP-InterRange.tex <==

\begin{table}[t]    
    \centering
    \caption{\textbf{Interaction range} --- All the values for effective interaction are given in ten-thousandth ($10^{-5}$). Influence tends to decrease over time for all kernels.}
    \label{tab-interRange}
    \begin{tabularx}{\textwidth}{|c|c|c|X|X|X|X|X|X|X|X|X|X|}
        \cline{1-12}
        $\vec{\kappa} (t)$ & $\theta_0$ & $r$ & $\kappa_1$ & $\kappa_2$ & $\kappa_3$ & $\kappa_4$ & $\kappa_5$ & $\kappa_6$ & $\kappa_7$ & $\kappa_8$ & $\kappa_9$ \\
        \cline{1-12}
        & & & 0m & 10m & 20m & 30m & 40m & 50m & 60m & 70m & 80m \\
        \cline{1-12}
        {\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Minute (m)}}}} & {\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{0.01}}}} & 0.5 & 133 & 421 & 407 & 451 & 428 & 403 & 395 & 345 & 121 \\
        & & 1 & 198 & 591 & 580 & 607 & 532 & 575 & 521 & 507 & 224 \\
        & & 1.5 & 308 & 937 & 893 & 914 & 955 & 840 & 808 & 810 & 304 \\
        \cdashline{2-12}
        & {\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{0.001}}}} & 0.5 & 218 & 509 & 457 & 424 & 371 & 340 & 313 & 178 & 52 \\
        & & 1 & 142 & 435 & 396 & 388 & 343 & 327 & 272 & 187 & 45 \\
        & & 1.5 & 104 & 388 & 366 & 353 & 326 & 333 & 290 & 215 & 61 \\
        \cline{1-12}
        
        % ==================
        
        & & & 0h & 2h & 4h & 6h & 8h & - & - & - & - \\
        \cline{1-12}
        {\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Hour (h)}}}} & {\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{0.01}}}} & 0.5 & 247 & 430 & 502 & 456 & 324 & & & & \\
        & & 1 & 329 & 538 & 549 & 542 & 451 & & & & \\
        & & 1.5 & 229 & 615 & 532 & 526 & 411 & & & & \\
        \cdashline{2-8}
        & {\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{0.001}}}} & 0.5 & 62 & 149 & 119 & 137 & 92 & & & & \\
        & & 1 & 77 & 164 & 172 & 149 & 111 & & & & \\
        & & 1.5 & 104 & 244 & 223 & 197 & 156 & & & & \\
        \cline{1-12}
        
        % ==================
        
        & & & 0d & 1d & 2d & 3d & 4d & 5d & 6d & - & - \\
        \cline{1-12}
        {\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Day (d)}}}} & {\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{0.01}}}} & 0.5 & 22 & 45 & 47 & 46 & 47 & 47 & 37 & & \\
        & & 1 & 35 & 71 & 72 & 68 & 68 & 70 & 61 & & \\
        & & 1.5 & 51 & 100 & 101 & 105 & 98 & 105 & 82 & & \\
        \cdashline{2-10}
        & {\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{0.001}}}} & 0.5 & 9 & 20 & 21 & 21 & 21 & 21 & 17 & & \\
        & & 1 & 12 & 26 & 24 & 27 & 28 & 26 & 22 & & \\
        & & 1.5 & 11 & 41 & 42 & 41 & 41 & 41 & 35 & & \\
        \cline{1-12}
        
         
    \end{tabularx}
\end{table}


==> table-MPDHP-fit.tex <==

\begin{table}[h]
    \centering    
    \caption{\textbf{Results for each experiment} --- We characterize each run in terms of clusters (number, size, textual entropy, subreddits entropy). The standard deviation on the last digits is given between parenthesis.}
    \label{tab-diffruns}
    \begin{tabularx}{\textwidth}{|>{\hsize=.25\hsize}X|>{\hsize=.25\hsize}X|>{\hsize=.5\hsize}X|X|X|X|X|}
        \cline{1-7}
        $\vec{\kappa} (t)$ & $\theta_0$ & $r$ & $K$ & $<N>$ & $S_{text}^{(20)}$ & $S_{sub}^{(20)}$ \\
        \cline{1-7}
        {\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{Minute}}}} & {\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{0.01}}}} & 0.0 & 16150 & 6 & 0.744(68) & 0.400(36) \\
        & & 0.5 & 8498 & 12 & 0.796(55) & 0.441(24) \\
        & & 1.0 & 5069 & 20 & 0.790(49) & 0.476(53) \\
        & & 1.5 & 2730 & 37 & 0.808(43) & 0.490(52) \\
        \cdashline{2-7}
        & {\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{0.001}}}} & 0.0 & 46304 & 2 & 0.475(48) & 0.239(56) \\
        & & 0.5 & 37277 & 3 & 0.485(40) & 0.256(60) \\
        & & 1.0 & 26858 & 4 & 0.501(37) & 0.266(72) \\
        & & 1.5 & 19275 & 5 & 0.506(39) & 0.280(58) \\
        \cline{1-7}
        
        % ========================
        
        {\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{Hour}}}} & {\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{0.01}}}} & 0.0 & 3792 & 27 & 0.798(52) & 0.474(106) \\
        & & 0.5 & 1735 & 59 & 0.791(45) & 0.469(77) \\
        & & 1.0 & 825 & 124 & 0.803(47) & 0.484(75) \\
        & & 1.5 & 426 & 240 & 0.795(37) & 0.489(69) \\
        \cdashline{2-7}
        & {\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{0.001}}}} & 0.0 & 18012 & 6 & 0.760(86) & 0.397(63) \\
        & & 0.5 & 11923 & 9 & 0.784(72) & 0.425(38) \\
        & & 1.0 & 4837 & 21 & 0.821(50) & 0.497(30) \\
        & & 1.5 & 2368 & 43 & 0.814(42) & 0.481(91) \\
        \cline{1-7}
        
        % ========================
        
        {\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{Day}}}} & {\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{0.01}}}} & 0.0 & 609 & 168 & 0.713(34) & 0.413(103) \\
        & & 0.5 & 326 & 313 & 0.728(33) & 0.429(98) \\
        & & 1.0 & 172 & 593 & 0.743(31) & 0.461(94) \\
        & & 1.5 & 96 & 1063 & 0.755(36) & 0.464(86) \\
        \cdashline{2-7}
        & {\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{0.001}}}} & 0.0 & 4349 & 23 & 0.705(49) & 0.396(103) \\
        & & 0.5 & 2654 & 38 & 0.721(59) & 0.404(104) \\
        & & 1.0 & 1399 & 73 & 0.734(57) & 0.431(106) \\
        & & 1.5 & 764 & 134 & 0.741(54) & 0.442(98) \\
        \cline{1-7}
         
    \end{tabularx}
\end{table}


==> table-MPDHP-interStrength.tex <==

\begin{table}[h]
    \centering
    \caption{\textbf{Interaction strength} --- Overall, interaction between clusters is weak. The standard deviation on the last digits are given between parenthesis. The large standard deviations suggest that there is a large variety of interacting behaviours. Interactions tend to happen within a cluster (self-interactions).
    }
    \label{tab-interStrength}
    \begin{tabularx}{\textwidth}{|c|c|c|X|X|X|X|}
        \cline{1-7}
        $\vec{\kappa} (t)$ & $\theta_0$ & $r$ & $<A>$ ($10^{-3}$) & $<W>$ ($10^{-5}$) & $<A>_W$ ($10^{-3}$) & $\frac{<W^{intra}>}{<W^{extra}>}$ \\
        \cline{1-7}
        {\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Minute}}}} & {\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{0.01}}}} & 0.5 & 49(21) & 342(889) & 66(17) & 1.8(62) \\
        & & 1.0 & 48(20) & 478(1124) & 60(17) & 1.4(43) \\
        & & 1.5 & 48(20) & 746(1901) & 60(17) & 1.0(33) \\
        \cdashline{2-7}
        & {\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{0.001}}}} & 0.5 & 50(22) & 316(882) & 66(17) & 3.1(138) \\
        & & 1.0 & 50(21) & 279(752) & 67(16) & 2.6(105) \\
        & & 1.5 & 50(22) & 268(665) & 67(16) & 2.3(84) \\
        \cline{1-7}
        
        % ========================
        
        {\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Hour}}}} & {\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{0.01}}}} & 0.5 & 49(18) & 389(843) & 56(17) & 0.5(13) \\
        & & 1.0 & 49(18) & 478(1187) & 56(17) & 0.6(15) \\
        & & 1.5 & 48(17) & 471(789) & 52(15) & 0.7(13) \\
        \cdashline{2-7}
        & {\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{0.001}}}} & 0.5 & 50(21) & 110(398) & 61(17) & 1.7(67) \\
        & & 1.0 & 50(18) & 133(506) & 57(17) & 1.4(60) \\
        & & 1.5 & 49(17) & 183(554) & 55(17) & 1.1(37) \\
        \cline{1-7}
        
        % ========================
        
        {\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Day}}}} & {\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{0.01}}}} & 0.5 & 49(18) & 41(97) & 55(17) & 1.2(34) \\
        & & 1.0 & 49(19) & 63(131) & 54(17) & 1.2(31) \\
        & & 1.5 & 49(19) & 91(187) & 53(18) & 1.2(31) \\
        \cdashline{2-7}
        & {\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{0.001}}}} & 0.5 & 50(20) & 18(90) & 60(19) & 1.1(59) \\
        & & 1.0 & 50(19) & 23(101) & 58(17) & 1.0(50) \\
        & & 1.5 & 50(19) & 37(111) & 56(18) & 1.0(36) \\
        \cline{1-7}
         
    \end{tabularx}
    
    
\end{table}

